MetaLDC: Meta Learning of Low-Dimensional Computing Classifiers for Fast On-Device Adaption

Fast model updates for unseen tasks on intelligent edge devices are crucial but also challenging due to the limited computational power. In this paper,we propose MetaLDC, which meta-trains braininspired ultra-efficient low-dimensional computing classifiers to enable fast adaptation on tiny devices with minimal computational costs. Concretely, during the meta-training stage, MetaLDC meta trains a representation offline by explicitly taking into account that the final (binary) class layer will be fine-tuned for fast adaptation for unseen tasks on tiny devices; during the meta-testing stage, MetaLDC uses closed-form gradients of the loss function to enable fast adaptation of the class layer. Unlike traditional neural networks, MetaLDC is designed based on the emerging LDC framework to enable ultra-efficient on-device inference. Our experiments have demonstrated that compared to SOTA baselines, MetaLDC achieves higher accuracy, robustness against random bit errors, as well as cost-efficient hardware computation.

==> contents/Tables/isolet.tex <==
\begin{table*}[h]
  
    \centering
    \begin{tabular}{lcccccc}
    \toprule
    & \multicolumn{5}{c}{\textbf{Evaluation Tasks}} \\
    \cmidrule{2-6}
    \textbf{Methods} &  $T_1$ &   $T_2$ &  $T_3$ &  $T_4$ &  $T_5$ & \textbf{Avg Acc}\\
    \midrule
     HDC w/ retraining & 79.17 & 83.31 & 78.74 & 81.01 & 85.48 & 81.54\\
    Pretrained LDC & 81.77 & 84.11& 79.01 & 83.92 & 87.63 & 85.29\\
    MAML LDC (full) & 83.81 & 87.97 & 82.06 & 85.97 & 89.89 & 85.94\\
    \textbf{MAML LDC (ours)} & \textbf{84.07} & \textbf{88.81} &  \textbf{82.18} & \textbf{86.11} & \textbf{90.11} & \textbf{86.26}\\
    \midrule
    Upper Bound (MAML MLP) & 91.67 & 92.78 & 89.07 & 92.45 & 93.78 & 91.95\\
    \bottomrule
    \end{tabular}
    \caption{Accuracy of our MAML LDC compared to other methods on the Split-ISOLET. The `MAML-' methods use $K=1$. }
    \label{tab:isolet1}
\end{table*}
